Vector boson fusion at NNLO in QCD: SM Higgs and beyond

Weak vector boson fusion provides a unique channel to directly probe the mechanism of electroweak symmetry breaking at hadron colliders. We present a method that allows to calculate total cross sections to next-to-next-to-leading order (NNLO) in QCD for an arbitrary V* V* -> X process, the so-called structure function approach. By discussing the case of Higgs production in detail, we estimate several classes of previously neglected contributions and we argue that such method is accurate at a precision level well above the typical residual scale and PDF uncertainties at NNLO. Predictions for cross sections at the Tevatron and the LHC are presented for a variety of cases: the Standard Model Higgs (including anomalous couplings), neutral and charged scalars in extended Higgs sectors and (fermiophobic) vector resonance production. Further results can be easily obtained through the public use of the VBF@NNLO code.

==> Tables/table-MSTW08-1960-sc1.tex <==
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|ccc|}
\hline $ M_h [\gev] $ & $ \sigma_{LO} $ & $ \sigma_{NLO} $ & $ \sigma_{NNLO} $ \\ \hline
$ 90 $ & $ 1.125 ^{+0.155+0.043} _{-0.125-0.043} \cdot 10^{-1} $ & $ 1.176 ^{+0.030+0.053} _{-0.023-0.053} \cdot 10^{-1} $ & $ 1.181 ^{+0.008+0.056} _{-0.003-0.056} \cdot 10^{-1} $ \\[1mm]
$ 95 $ & $ 1.035 ^{+0.146+0.040} _{-0.117-0.040} \cdot 10^{-1} $ & $ 1.081 ^{+0.027+0.049} _{-0.021-0.049} \cdot 10^{-1} $ & $ 1.087 ^{+0.008+0.052} _{-0.002-0.052} \cdot 10^{-1} $ \\[1mm]
$ 100 $ & $ 9.533 ^{+1.381+0.368} _{-1.097-0.368} \cdot 10^{-2} $ & $ 9.950 ^{+0.282+0.453} _{-0.195-0.453} \cdot 10^{-2} $ & $ 1.001 ^{+0.007+0.048} _{-0.003-0.048} \cdot 10^{-1} $ \\[1mm]
$ 105 $ & $ 8.791 ^{+1.299+0.342} _{-1.027-0.342} \cdot 10^{-2} $ & $ 9.176 ^{+0.239+0.420} _{-0.191-0.420} \cdot 10^{-2} $ & $ 9.231 ^{+0.061+0.449} _{-0.028-0.449} \cdot 10^{-2} $ \\[1mm]
$ 110 $ & $ 8.111 ^{+1.224+0.318} _{-0.969-0.318} \cdot 10^{-2} $ & $ 8.461 ^{+0.228+0.390} _{-0.187-0.390} \cdot 10^{-2} $ & $ 8.514 ^{+0.064+0.416} _{-0.025-0.416} \cdot 10^{-2} $ \\[1mm]
$ 115 $ & $ 7.488 ^{+1.154+0.295} _{-0.906-0.295} \cdot 10^{-2} $ & $ 7.806 ^{+0.225+0.362} _{-0.176-0.362} \cdot 10^{-2} $ & $ 7.861 ^{+0.059+0.386} _{-0.021-0.386} \cdot 10^{-2} $ \\[1mm]
$ 120 $ & $ 6.920 ^{+1.083+0.274} _{-0.851-0.274} \cdot 10^{-2} $ & $ 7.213 ^{+0.196+0.336} _{-0.172-0.336} \cdot 10^{-2} $ & $ 7.267 ^{+0.046+0.359} _{-0.026-0.359} \cdot 10^{-2} $ \\[1mm]
$ 125 $ & $ 6.396 ^{+1.019+0.255} _{-0.798-0.255} \cdot 10^{-2} $ & $ 6.666 ^{+0.178+0.312} _{-0.145-0.312} \cdot 10^{-2} $ & $ 6.713 ^{+0.047+0.333} _{-0.020-0.333} \cdot 10^{-2} $ \\[1mm]
$ 130 $ & $ 5.918 ^{+0.959+0.238} _{-0.750-0.238} \cdot 10^{-2} $ & $ 6.168 ^{+0.173+0.290} _{-0.153-0.290} \cdot 10^{-2} $ & $ 6.213 ^{+0.043+0.310} _{-0.026-0.310} \cdot 10^{-2} $ \\[1mm]
$ 135 $ & $ 5.479 ^{+0.903+0.221} _{-0.703-0.221} \cdot 10^{-2} $ & $ 5.705 ^{+0.160+0.270} _{-0.147-0.270} \cdot 10^{-2} $ & $ 5.751 ^{+0.040+0.288} _{-0.024-0.288} \cdot 10^{-2} $ \\[1mm]
$ 140 $ & $ 5.079 ^{+0.847+0.206} _{-0.662-0.206} \cdot 10^{-2} $ & $ 5.283 ^{+0.153+0.251} _{-0.138-0.251} \cdot 10^{-2} $ & $ 5.325 ^{+0.037+0.268} _{-0.022-0.268} \cdot 10^{-2} $ \\[1mm]
$ 145 $ & $ 4.706 ^{+0.798+0.192} _{-0.622-0.192} \cdot 10^{-2} $ & $ 4.896 ^{+0.140+0.234} _{-0.132-0.234} \cdot 10^{-2} $ & $ 4.936 ^{+0.034+0.250} _{-0.021-0.250} \cdot 10^{-2} $ \\[1mm]
$ 150 $ & $ 4.362 ^{+0.755+0.179} _{-0.583-0.179} \cdot 10^{-2} $ & $ 4.539 ^{+0.131+0.218} _{-0.125-0.218} \cdot 10^{-2} $ & $ 4.575 ^{+0.034+0.232} _{-0.021-0.232} \cdot 10^{-2} $ \\[1mm]
$ 155 $ & $ 4.046 ^{+0.713+0.167} _{-0.545-0.167} \cdot 10^{-2} $ & $ 4.207 ^{+0.124+0.203} _{-0.118-0.203} \cdot 10^{-2} $ & $ 4.244 ^{+0.032+0.217} _{-0.020-0.217} \cdot 10^{-2} $ \\[1mm]
$ 160 $ & $ 3.759 ^{+0.670+0.156} _{-0.513-0.156} \cdot 10^{-2} $ & $ 3.906 ^{+0.116+0.189} _{-0.114-0.189} \cdot 10^{-2} $ & $ 3.940 ^{+0.028+0.202} _{-0.019-0.202} \cdot 10^{-2} $ \\[1mm]
$ 165 $ & $ 3.492 ^{+0.630+0.145} _{-0.484-0.145} \cdot 10^{-2} $ & $ 3.627 ^{+0.108+0.176} _{-0.108-0.176} \cdot 10^{-2} $ & $ 3.659 ^{+0.026+0.188} _{-0.020-0.188} \cdot 10^{-2} $ \\[1mm]
$ 170 $ & $ 3.244 ^{+0.592+0.136} _{-0.454-0.136} \cdot 10^{-2} $ & $ 3.368 ^{+0.101+0.164} _{-0.103-0.164} \cdot 10^{-2} $ & $ 3.399 ^{+0.023+0.175} _{-0.019-0.175} \cdot 10^{-2} $ \\[1mm]
$ 175 $ & $ 3.016 ^{+0.559+0.127} _{-0.426-0.127} \cdot 10^{-2} $ & $ 3.130 ^{+0.095+0.153} _{-0.098-0.153} \cdot 10^{-2} $ & $ 3.159 ^{+0.023+0.164} _{-0.018-0.164} \cdot 10^{-2} $ \\[1mm]
$ 180 $ & $ 2.805 ^{+0.524+0.118} _{-0.400-0.118} \cdot 10^{-2} $ & $ 2.910 ^{+0.088+0.143} _{-0.094-0.143} \cdot 10^{-2} $ & $ 2.937 ^{+0.022+0.153} _{-0.017-0.153} \cdot 10^{-2} $ \\[1mm]
$ 185 $ & $ 2.610 ^{+0.495+0.111} _{-0.376-0.111} \cdot 10^{-2} $ & $ 2.707 ^{+0.083+0.134} _{-0.088-0.134} \cdot 10^{-2} $ & $ 2.732 ^{+0.020+0.143} _{-0.017-0.143} \cdot 10^{-2} $ \\[1mm]
$ 190 $ & $ 2.429 ^{+0.465+0.103} _{-0.353-0.103} \cdot 10^{-2} $ & $ 2.519 ^{+0.078+0.125} _{-0.084-0.125} \cdot 10^{-2} $ & $ 2.542 ^{+0.019+0.133} _{-0.016-0.133} \cdot 10^{-2} $ \\[1mm]
$ 195 $ & $ 2.262 ^{+0.438+0.097} _{-0.333-0.097} \cdot 10^{-2} $ & $ 2.344 ^{+0.075+0.117} _{-0.080-0.117} \cdot 10^{-2} $ & $ 2.367 ^{+0.018+0.124} _{-0.015-0.124} \cdot 10^{-2} $ \\[1mm]
$ 200 $ & $ 2.107 ^{+0.413+0.090} _{-0.313-0.090} \cdot 10^{-2} $ & $ 2.183 ^{+0.071+0.109} _{-0.075-0.109} \cdot 10^{-2} $ & $ 2.205 ^{+0.017+0.116} _{-0.015-0.116} \cdot 10^{-2} $ \\[1mm]
$ 210 $ & $ 1.830 ^{+0.368+0.079} _{-0.276-0.079} \cdot 10^{-2} $ & $ 1.896 ^{+0.059+0.095} _{-0.069-0.095} \cdot 10^{-2} $ & $ 1.914 ^{+0.014+0.102} _{-0.014-0.102} \cdot 10^{-2} $ \\[1mm]
$ 220 $ & $ 1.591 ^{+0.327+0.069} _{-0.244-0.069} \cdot 10^{-2} $ & $ 1.648 ^{+0.054+0.084} _{-0.063-0.084} \cdot 10^{-2} $ & $ 1.665 ^{+0.012+0.089} _{-0.013-0.089} \cdot 10^{-2} $ \\[1mm]
$ 230 $ & $ 1.386 ^{+0.291+0.061} _{-0.217-0.061} \cdot 10^{-2} $ & $ 1.434 ^{+0.048+0.073} _{-0.056-0.073} \cdot 10^{-2} $ & $ 1.449 ^{+0.011+0.078} _{-0.012-0.078} \cdot 10^{-2} $ \\[1mm]
$ 240 $ & $ 1.208 ^{+0.259+0.053} _{-0.192-0.053} \cdot 10^{-2} $ & $ 1.249 ^{+0.042+0.064} _{-0.051-0.064} \cdot 10^{-2} $ & $ 1.262 ^{+0.010+0.068} _{-0.011-0.068} \cdot 10^{-2} $ \\[1mm]
$ 250 $ & $ 1.054 ^{+0.230+0.047} _{-0.170-0.047} \cdot 10^{-2} $ & $ 1.089 ^{+0.038+0.056} _{-0.046-0.056} \cdot 10^{-2} $ & $ 1.101 ^{+0.009+0.060} _{-0.010-0.060} \cdot 10^{-2} $ \\[1mm]
$ 260 $ & $ 9.210 ^{+2.047+0.412} _{-1.510-0.412} \cdot 10^{-3} $ & $ 9.510 ^{+0.333+0.495} _{-0.410-0.495} \cdot 10^{-3} $ & $ 9.618 ^{+0.074+0.526} _{-0.093-0.526} \cdot 10^{-3} $ \\[1mm]
$ 270 $ & $ 8.052 ^{+1.827+0.363} _{-1.339-0.363} \cdot 10^{-3} $ & $ 8.309 ^{+0.296+0.435} _{-0.370-0.435} \cdot 10^{-3} $ & $ 8.406 ^{+0.066+0.462} _{-0.083-0.462} \cdot 10^{-3} $ \\[1mm]
$ 280 $ & $ 7.047 ^{+1.622+0.319} _{-1.188-0.319} \cdot 10^{-3} $ & $ 7.269 ^{+0.261+0.383} _{-0.334-0.383} \cdot 10^{-3} $ & $ 7.353 ^{+0.060+0.406} _{-0.078-0.406} \cdot 10^{-3} $ \\[1mm]
$ 290 $ & $ 6.170 ^{+1.448+0.281} _{-1.054-0.281} \cdot 10^{-3} $ & $ 6.362 ^{+0.233+0.337} _{-0.301-0.337} \cdot 10^{-3} $ & $ 6.439 ^{+0.052+0.358} _{-0.072-0.358} \cdot 10^{-3} $ \\[1mm]
$ 300 $ & $ 5.406 ^{+1.296+0.248} _{-0.935-0.248} \cdot 10^{-3} $ & $ 5.571 ^{+0.207+0.297} _{-0.271-0.297} \cdot 10^{-3} $ & $ 5.639 ^{+0.046+0.315} _{-0.062-0.315} \cdot 10^{-3} $ \\[1mm]
\hline
\end{tabular}
\caption{
\small 
Total LO, NLO, NNLO VBF cross-section at the Tevatron, $\sqrt S = 1.96 \tev$. Errors shown are respectively scale and PDF uncertainities. Scale uncertainities are evaluated by varying the renormalization and factorization scales in the interval $ 1/2 Q^2 < \mu_r, \mu_f < 2 Q^2 $. The MSTW2008~\cite{Martin:2009iq} PDF set has been used. PDF errors are at 90\% CL.}
\label{tab:xsect-1960-sc-1}
\end{center}
\end{table}


==> Tables/table_tbloops_Tev_sqrts1960.tex <==
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|ccccc|}
\hline $ \hmass \,[\gev] $ & $ \sigma_{\rm{LO}} $ & $ \sigma_{ \rm{tri}+\rm{box} } $ & $ \sigma_{ \rm{tri} } $ & $ \sigma_{ \rm{box} } $ & $ \sigma_{ \rm{tri}+\rm{box} } ^{\infty} $ \\ \hline
$  100 $ & $ 8.80 \cdot 10^{-2} $ & $ 6.64 \cdot 10^{-6} $ & $ 4.33 \cdot 10^{-6} $ & $ 1.05 \cdot 10^{-6} $ & $ 6.11 \cdot 10^{-6} $ \\
$  120 $ & $ 6.38 \cdot 10^{-2} $ & $ 5.43 \cdot 10^{-6} $ & $ 3.40 \cdot 10^{-6} $ & $ 9.82 \cdot 10^{-7} $ & $ 4.78 \cdot 10^{-6} $ \\
$  150 $ & $ 4.01 \cdot 10^{-2} $ & $ 4.01 \cdot 10^{-6} $ & $ 2.35 \cdot 10^{-6} $ & $ 8.78 \cdot 10^{-7} $ & $ 3.31 \cdot 10^{-6} $ \\
$  200 $ & $ 1.93 \cdot 10^{-2} $ & $ 2.40 \cdot 10^{-6} $ & $ 1.28 \cdot 10^{-6} $ & $ 6.81 \cdot 10^{-7} $ & $ 1.81 \cdot 10^{-6} $ \\
$  250 $ & $ 9.64 \cdot 10^{-3} $ & $ 1.33 \cdot 10^{-6} $ & $ 6.94 \cdot 10^{-7} $ & $ 4.66 \cdot 10^{-7} $ & $ 9.95 \cdot 10^{-7} $ \\
$  300 $ & $ 4.94 \cdot 10^{-3} $ & $ 6.16 \cdot 10^{-7} $ & $ 3.77 \cdot 10^{-7} $ & $ 2.61 \cdot 10^{-7} $ & $ 5.48 \cdot 10^{-7} $ \\
\hline
\end{tabular}
\caption{\small
Values of the contributions to the total NNLO VBF cross-section due to the heavy-quark loop diagrams shown in \cf{fig:heavyquarks} at the Tevatron, $\sqrt S = 1.96 \tev$. The MSTW2008~\cite{Martin:2009iq} NNLO PDF set has been used.  The LO cross-section, computed with LO PDFs, is also shown for comparison. Renormalization and factorization scales have been set to $\wmass$. Integration errors are below the 1\% level. Cross-sections are in pb.}
\label{tab:tbloops-1960}
\end{center}
\end{table}


==> Tables/table_tbloops_tri-glu_Tev_sqrts1960.tex <==
\begin{tabular}{|c|cc|}
\hline $ \hmass\, [\gev] $ & $ \sigma_{LO} $ & $  \sigma_{\rm{tri}}^{ 1 \, \rm{loop+glu}} $ \\ \hline
$  100 $ & $ 8.80 \cdot 10^{-2} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
$  120 $ & $ 6.38 \cdot 10^{-2} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
$  150 $ & $ 4.01 \cdot 10^{-2} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
$  200 $ & $ 1.93 \cdot 10^{-2} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
$  250 $ & $ 9.64 \cdot 10^{-3} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
$  300 $ & $ 4.94 \cdot 10^{-3} $ & $ 0.00 \cdot 10^{-2147483648} $ \\
\hline
\end{tabular}


==> Tables/table_tbloops_tri2loop_Tev_sqrts1960.tex <==
\begin{tabular}{|c|cc|}
\hline $ \hmass\, [\gev] $ & $ \sigma_{LO} $ & $  \sigma_{\rm{tri}}^{ 2\, \rm{loop}} $ \\ \hline
$  100 $ & $ 8.80 \cdot 10^{-2} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
$  120 $ & $ 6.38 \cdot 10^{-2} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
$  150 $ & $ 4.01 \cdot 10^{-2} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
$  200 $ & $ 1.93 \cdot 10^{-2} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
$  250 $ & $ 9.64 \cdot 10^{-3} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
$  300 $ & $ 4.94 \cdot 10^{-3} $ & $ -0.00 \cdot 10^{-2147483648} $ \\
\hline
\end{tabular}


==> Tables/table_tbloops_tri_LHC_sqrts14000.tex <==
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|cccc|}
\hline $ M_h [\gev] $ & $ \left| \rm{tri}_{ 2 \rm{ loops}}|^2 $ \\ \hline
$  100 $ & $ 2.300 \cdot 10^{-3} $ & $ 2.300 \cdot 10^{-3} $ \\
$  120 $ & $ 2.012 \cdot 10^{-3} $ & $ 2.012 \cdot 10^{-3} $ \\
$  150 $ & $ 1.665 \cdot 10^{-3} $ & $ 1.665 \cdot 10^{-3} $ \\
$  200 $ & $ 1.246 \cdot 10^{-3} $ & $ 1.246 \cdot 10^{-3} $ \\
$  250 $ & $ 9.628 \cdot 10^{-4} $ & $ 9.628 \cdot 10^{-4} $ \\
$  300 $ & $ 7.604 \cdot 10^{-4} $ & $ 7.604 \cdot 10^{-4} $ \\
$  400 $ & $ 4.985 \cdot 10^{-4} $ & $ 4.985 \cdot 10^{-4} $ \\
$  500 $ & $ 3.442 \cdot 10^{-4} $ & $ 3.442 \cdot 10^{-4} $ \\
$  650 $ & $ 2.098 \cdot 10^{-4} $ & $ 2.098 \cdot 10^{-4} $ \\
$  800 $ & $ 1.347 \cdot 10^{-4} $ & $ 1.347 \cdot 10^{-4} $ \\
$ 1000 $ & $ 7.906 \cdot 10^{-5} $ & $ 7.906 \cdot 10^{-5} $ \\
\hline
\end{tabular}
\caption{\small
Values of the contributions to the total NNLO VBF cross-section due to the heavy-quark two-loop trinagle shown in \cf{fig:heavyquarks-tri2loop} at the LHC, $\sqrt S = 14 \tev$. The MSTW2008~\cite{Martin:2009iq} NNLO PDF set has been used. Renormalization and factorization scales have been set to $M_W$. Integration errors are below the 1\% level. Numbers are in pb.}
\label{tab:tbloops-14000}
\end{center}
\end{table}


==> Tables/table_tbloops_tri_LHC_sqrts7000.tex <==
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|cccc|}
\hline $ M_h [\gev] $ & $ \left| \rm{tri}_{ 2 \rm{ loops}}|^2 $ \\ \hline
$  100 $ & $ 8.378 \cdot 10^{-4} $ & $ 8.378 \cdot 10^{-4} $ \\
$  120 $ & $ 7.079 \cdot 10^{-4} $ & $ 7.079 \cdot 10^{-4} $ \\
$  150 $ & $ 5.605 \cdot 10^{-4} $ & $ 5.605 \cdot 10^{-4} $ \\
$  200 $ & $ 3.905 \cdot 10^{-4} $ & $ 3.905 \cdot 10^{-4} $ \\
$  250 $ & $ 2.805 \cdot 10^{-4} $ & $ 2.805 \cdot 10^{-4} $ \\
$  300 $ & $ 2.064 \cdot 10^{-4} $ & $ 2.064 \cdot 10^{-4} $ \\
$  400 $ & $ 1.179 \cdot 10^{-4} $ & $ 1.179 \cdot 10^{-4} $ \\
$  500 $ & $ 7.083 \cdot 10^{-5} $ & $ 7.083 \cdot 10^{-5} $ \\
$  650 $ & $ 3.521 \cdot 10^{-5} $ & $ 3.521 \cdot 10^{-5} $ \\
$  800 $ & $ 1.842 \cdot 10^{-5} $ & $ 1.842 \cdot 10^{-5} $ \\
$ 1000 $ & $ 8.178 \cdot 10^{-6} $ & $ 8.178 \cdot 10^{-6} $ \\
\hline
\end{tabular}
\caption{\small
Values of the contributions to the total NNLO VBF cross-section due to the heavy-quark two-loop trinagle shown in \cf{fig:heavyquarks-tri2loop} at the LHC, $\sqrt S = 7 \tev$. The MSTW2008~\cite{Martin:2009iq} NNLO PDF set has been used. Renormalization and factorization scales have been set to $M_W$. Integration errors are below the 1\% level. Numbers are in pb.}
\label{tab:tbloops-7000}
\end{center}
\end{table}


==> Tables/table_tbloops_tri_Tev_sqrts1960.tex <==
\begin{table}[ht!]
\begin{center}
\begin{tabular}{|c|cccc|}
\hline $ M_h [\gev] $ & $ \left| \rm{tri}_{ 2 \rm{ loops}}|^2 $ \\ \hline
$  100 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
$  120 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
$  150 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
$  200 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
$  250 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
$  300 $ & $ -0.000 \cdot 10^{-2147483648} $ & $ -0.000 \cdot 10^{-2147483648} $ \\
\hline
\end{tabular}
\caption{\small
Values of the contributions to the total NNLO VBF cross-section due to the heavy-quark two-loop trinagle shown in \cf{fig:heavyquarks-tri2loop} at the Tevatron, $\sqrt S = 1.96 \tev$. The MSTW2008~\cite{Martin:2009iq} NNLO PDF set has been used. Renormalization and factorization scales have been set to $M_W$. Integration errors are below the 1\% level. Numbers are in pb.}
\label{tab:tbloops-1960}
\end{center}
\end{table}

